Rethinking Pseudo-Label Guided Learning for Weakly Supervised Temporal Action Localization from the Perspective of Noise Correction

Pseudo-label learning methods have been widely applied in weakly-supervised temporal action localization. Existing works directly utilize weakly-supervised base model to generate instance-level pseudo-labels for training the fully-supervised detection head. We argue that the noise in pseudo-labels would interfere with the learning of fully-supervised detection head, leading to significant performance leakage. Issues with noisy labels include:(1) inaccurate boundary localization; (2) undetected short action clips; (3) multiple adjacent segments incorrectly detected as one segment. To target these issues, we introduce a two-stage noisy label learning strategy to harness every potential useful signal in noisy labels. First, we propose a frame-level pseudo-label generation model with a context-aware denoising algorithm to refine the boundaries. Second, we introduce an online-revised teacher-student framework with a missing instance compensation module and an ambiguous instance correction module to solve the short-action-missing and many-to-one problems. Besides, we apply a high-quality pseudo-label mining loss in our online-revised teacher-student framework to add different weights to the noisy labels to train more effectively. Our model outperforms the previous state-of-the-art method in detection accuracy and inference speed greatly upon the THUMOS14 and ActivityNet v1.2 benchmarks.

==> table/Comparisons.tex <==
\begin{table*}[htb]
    \centering
    \renewcommand
    \arraystretch{1.2}
    \caption{Comparisons with state-of-the-art methods. AVG is the average mAP under the IoU thresholds 0.1:0.7:0.1 for THUMOS14 dataset. ’-’ means that the corresponding results are nor reported in the original papers. The best results are bold. The baselines are underlined.}
    \resizebox{470pt}{!}{

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}


\begin{tabular}{c|cc|ccccccc|ccc}
    \hline
    \multirow{2}{*}{\textbf{Sup.}}    & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Pub.}} & \multicolumn{7}{c|}{\textbf{mAP@IoU(\%)}}                                                                     & \multicolumn{3}{c}{\textbf{AVG mAP*(\%)}}     \\ \cline{4-13} 
                                      &                                  &                                & 0.1           & 0.2           & 0.3           & 0.4           & 0.5           & 0.6           & 0.7           & 0.1:0.5       & 0.3:0.7       & 0.1:0.7       \\ \hline
    \multirow{3}{*}{\textbf{Fully}}   & SSN \cite{zhao2017temporal}      & ICCV 2017                       & 60.3          & 56.2          & 50.6          & 40.8          & 29.1          & -             & -             & 47.4          & -             & -             \\
                                      & BSN\cite{lin2018bsn}             & ECCV 2018                       & 53.5          & 45.0            & 36.9          & 28.4          & 20.0            & -             & -             & 36.8          & -             & -             \\
                                      & TAL-Net \cite{chao2018rethinking}   & CVPR 2018                       & 59.8          & 57.1          & 53.2          & 48.5          & 42.8          & 33.8          & 20.8          & 52.3          & 39.8          & 45.1          \\ \hline
    \multirow{20}{*}{\textbf{Weakly}} & UGCT \cite{yang2021uncertainty}                     & CVPR 2021                       & 69.2          & 62.9          & 55.5          & 46.5          & 35.9          & 23.8          & 11.4          & 54.0            & 34.6          & 43.6          \\
                                      & CoLA \cite{zhang2021cola}                     & CVPR 2021                       & 66.2          & 59.5          & 51.5          & 41.9          & 32.2          & 22            & 13.1          & 50.3          & 32.1          & 40.9          \\
                                      & DCC \cite{li2022exploring}             & CVPR 2022                       & 69.0            & 63.8          & 55.9          & 45.9          & 35.7          & 24.3          & 13.7          & 54.1          & 35.1          & 44.0            \\
                                      & ECM \cite{zhao2022equivalent}        & TPAMI 2022                      & 62.6          & 55.1          & 46.5          & 38.2          & 29.1          & 19.5          & 10.9          & 46.3          & 28.8          & 37.4          \\
                                      &DELU \cite{chen2022dual}        & ECCV 2022                       & 71.5          & 66.2          & 56.5          & 47.7          & 40.5          & 27.2          & 15.3          & 56.5          & 37.4          & 46.4          \\
                                      & AICL \cite{li2023actionness}          & AAAI 2023                       & 73.1          & 67.8          & 58.2          & 48.7          & 36.9          & 25.3          & 14.9          & 56.9          & 36.8          & 46.4          \\
                                      & Wang et al. \cite{wang2023two}             & CVPR 2023                       & 73.0            & 68.2          & 60.0            & 47.9          & 37.1          & 24.4          & 12.7          & 57.2          & 36.4          & 46.2          \\
                                      & Li et al. \cite{li2023boosting}                   & CVPR 2023                       & 71.1          & 65.0            & 56.2          & 47.8          & 39.3          & 27.5          & 15.2          & 55.9          & 37.2          & 46.0            \\
                                      & Ren et al.\cite{ren2023proposal}                  & CVPR 2023                       & 71.8          & 67.5          & 58.9          & 49.0            & 40.0            & 27.1          & 15.1          & 57.4          & 38.0            & 47.1          \\
                                      &STCL-Net \cite{fu2023semantic}               & TPAMI 2023                      & 72.7          & 67.1          & 58.2          & 49.7          & 41.8          & 28.7          & 16.0            & 57.9          & 38.9          & 47.7          \\
                                      &Zhou et al. \cite{zhou2023improving}               & CVPR 2033                       & 74.0            & 69.4          & 60.7          & 51.8          & 42.7          & 26.2          & 13.1          & 59.7          & 38.9          & 48.3          \\
                                      &Ju et al. \cite{ju2023distilling}          & CVPR 2023                       & 73.5          & 68.8          & 61.5          & 53.8          & 42.0            & 29.4          & 16.8          & 59.9          & 40.7          & 49.4          \\
                                      & PivoTAL \cite{rizve2023pivotal}                 & CVPR 2023                       & 74.1          & 69.6          & 61.7          & 52.1          & 42.8          & 30.6          & 16.7          & 60.1          & 40.8          & 49.7          \\
                                      & AHLM  \cite{wang2023weakly}                 & ICCV 2023                       & 75.1          & 68.9          & 60.2          & 48.9          & 38.3          & 26.8          & 14.7          & 58.3          & 37.8          & 47.6          \\
                                      & CASE   \cite{liu2023revisiting}                 & ICCV 2023                       & 72.3          & 67.1          & 59.2          & 49.4          & 37.7          & 24.2          & 13.7          & 57.1          & 36.8          & 46.2          \\
                                      & DDG-Net\cite{tang2023ddg}               & ICCV 2023                       & 72.5          & 67.7          & 58.2          & 49            & 41.4          & 27.6          & 14.8          & 57.8          & 38.2          & 47.3          \\ 
                                      
                                      \cdashline{2-13}[5pt/1pt]
                                      & \underline{ \textbf{CO$_2$-Net \cite{hong2021cross}}}         & \textbf{ACM MM 2021}            & \textbf{70.1} & \textbf{63.6} & \textbf{54.5} & \textbf{45.7} & \textbf{38.3} & \textbf{26.4} & \textbf{13.4} & \textbf{54.4} & \textbf{35.7} & \textbf{44.6} \\
                                      & \textbf{CO2-Net+NoCo}            & \textbf{-}                     & \textbf{74.6} & \textbf{70.3} & \textbf{63.0}   & \textbf{53.9} & \textbf{44.0}   & \textbf{31.7} & \textbf{17.4} & \textbf{61.2} & \textbf{42.0}   & \textbf{50.7} \\ 
                                      \cdashline{2-13}[5pt/1pt]
                                      & \underline{\textbf{ASM-Loc \cite{he2022asm}}}       & \textbf{CVPR 2022}              & \textbf{71.2} & \textbf{65.5} & \textbf{57.1} & \textbf{46.8} & \textbf{36.6} & \textbf{25.2} & \textbf{13.4} & \textbf{55.4} & \textbf{35.8} & \textbf{45.1} \\
                                      & \textbf{ASM-Loc+NoCo}            & \textbf{-}                     & \textbf{75.2} & \textbf{70.7} & \textbf{63.0}   & \textbf{54.1} & \textbf{44.0}   & \textbf{31.7} & \textbf{17.7} & \textbf{61.4} & \textbf{42.1} & \textbf{50.9} \\ \hline
    \end{tabular}
    
    
    
    
    
    }
    \label{new-table1}
    \end{table*}

==> table/DetectionResults.tex <==
% \begin{table*}[htb]
%     \centering
%     \renewcommand\arraystretch{1.2}
%     \caption{new-table2}
%     \resizebox{\linewidth}{!}{
    
%     \begin{tabular}{c|cc|cccc}
%     \hline
%     \multirow{2}{*}{\textbf{Sup.}}    & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Pub.}} & \multicolumn{4}{c}{\textbf{mAP@IoU(\%)}}                     \\
%                                       &                                  &                                & 0.5           & 0.75          & 0.95         & AVG           \\
%                                        \hline
%     \textbf{Fully}                    &  SSN \cite{zhao2017temporal}                   & ICCV 2017                       & 41.3          & 27            & 6.1          & 26.6          \\ 
%     \hline
%     \multirow{18}{*}{\textbf{Weakly}} & EM-MIL{[}13{]}                   & ECCV 2020                       & 37.4          & 23.1          & 2            & 20.3          \\
%                                       & MSA-Net{[}33{]}    MSA-Net \cite{yang2021multi}               & TIP 2021                        & 43.4          & 28.4          & 5.6          & 25.7          \\
%                                       & CoLA{[}36{]}                     & CVPR 2021                       & 42.7          & 25.7          & 5.8          & 26.1          \\
%                                       & HAM-Net{[}47{]}                  & AAAI 2021                       & 41            & 24.8          & 5.3          & 25.1          \\
%                                       &  AUMN \cite{luo2021action}                    & CVPR 2021                       & 42            & 25            & 5.6          & 25.5          \\
%                                       & D2-Net{[}9{]}                    & ICCV 2021                       & 42.3          & 25.5          & 5.8          & 26            \\
%                                       &  ECM \cite{zhao2022equivalent}                & TPAMI 2022                      & 41            & 24.9          & 6.5          & 25.5          \\
%                                       & DELU \cite{chen2022dual}           & ECCV 2022                       & 44.2          & 26.7          & 5.4          & 26.9          \\
%                                       &AICL \cite{li2023actionness}                    & AAAI 2023                       & 49.6          & 29.1          & 5.9          & 29.9          \\
%                                       & Ren et al.{[}40{]}               & CVPR 2023                       & 44.2          & 26.1          & 5.3          & 25.5          \\
%                                       & STCL-Net{[}4{]}                  & TPAMI 2023                      & 44            & 26.1          & 5.3          & 26.6          \\
%                                       & Ju et al.{[}42{]}                & CVPR 2023                       & 48.3          & 29.3          & 6.1          & 29.6          \\
%                                       & DDG-Net{[}44{]}                  & ICCV 2023                       & 44.3          & 26.9          & 5.5          & 27            \\
%                                       & CASE{[}43{]}                     & ICCV 2023                       & 43.8          & 27.2          & 6.7          & 27.9          \\
%                                       \cdashline{2-7}[5pt/1pt]
%                                       & \textbf{CO2-Net{[}45{]}}         & \textbf{ACM MM 2021}           & \textbf{43.3} & \textbf{26.3} & \textbf{5.2} & \textbf{26.4} \\
%                                       & \textbf{CO2-Net+NoCo}            & \textbf{-}                     & \textbf{48.9} & \textbf{30}   & \textbf{6.6} & \textbf{30.1} \\
%                                       \cdashline{2-7}[5pt/1pt]
%                                       & \textbf{ASM-Loc{[}46{]}}         & \textbf{CVPR 2022}              & \textbf{43.4} & \textbf{26.6} & \textbf{5.3} & \textbf{26.5} \\
%                                       & \textbf{ASM-Loc+NoCo}            & \textbf{-}                     & \textbf{49.1} & \textbf{30.5} & \textbf{6.7} & \textbf{30.7} \\ 
%                                       \hline
%     \end{tabular}
    
    
%     }
%     \label{new-table2}
%     \end{table*}


\begin{table}[htb]
\centering
\caption{Detection results on ActivityNet1.2 in terms of mAP@{0.5, 0.7, 0.9} and average mAP at tIoU thresholds $\alpha \in (0.5, 0.95)$ with step 0.05 (in percentage). It shows both fully-supervised method and weakly-supervised ones.}
\renewcommand\arraystretch{1.2}
\resizebox{\linewidth}{!}{
    \begin{tabular}{c|cc|cccc}
    \hline
    \multirow{2}{*}{\textbf{Sup.}}    & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Pub.}} & \multicolumn{4}{c}{\textbf{mAP@IoU(\%)}}                     \\
                                      &                                  &                                & 0.5           & 0.75          & 0.95         & AVG           \\
                                       \hline
    \textbf{Fully}                    &  SSN \cite{zhao2017temporal}                   & ICCV 2017                       & 41.3          & 27.0            & 6.1          & 26.6          \\ 
    \hline
    \multirow{18}{*}{\textbf{Weakly}} & EM-MIL \cite{luo2020weakly}                   & ECCV 2020                       & 37.4          & 23.1          & 2.0            & 20.3          \\
                                      & MSA-Net \cite{yang2021multi}               & TIP 2021                        & 43.4          & 28.4          & 5.6          & 25.7          \\
                                      & CoLA \cite{zhang2021cola}                     & CVPR 2021                       & 42.7          & 25.7          & 5.8          & 26.1          \\
                                      & HAM-Net \cite{islam2021hybrid}                  & AAAI 2021                       & 41.0            & 24.8          & 5.3          & 25.1          \\
                                      &  AUMN \cite{luo2021action}                    & CVPR 2021                       & 42.0            & 25.0            & 5.6          & 25.5          \\
                                      & D2-Net \cite{narayan2021d2}                    & ICCV 2021                       & 42.3          & 25.5          & 5.8          & 26.0            \\
                                      &  ECM \cite{zhao2022equivalent}                & TPAMI 2022                      & 41.0            & 24.9          & 6.5          & 25.5          \\
                                      & DELU \cite{chen2022dual}           & ECCV 2022                       & 44.2          & 26.7          & 5.4          & 26.9          \\
                                      &AICL \cite{li2023actionness}                    & AAAI 2023                       & 49.6          & 29.1          & 5.9          & 29.9          \\
                                      & Ren et al.\cite{ren2023proposal}               & CVPR 2023                       & 44.2          & 26.1          & 5.3          & 25.5          \\
                                      & STCL-Net \cite{fu2023semantic}               & TPAMI 2023                      & 44.0            & 26.1          & 5.3          & 26.6          \\
                                      & Ju et al. \cite{ju2023distilling}                & CVPR 2023                       & 48.3          & 29.3          & 6.1          & 29.6          \\
                                      & DDG-Net \cite{tang2023ddg}                & ICCV 2023                       & 44.3          & 26.9          & 5.5          & 27.0            \\
                                      & CASE \cite{liu2023revisiting}                    & ICCV 2023                       & 43.8          & 27.2          & 6.7          & 27.9          \\
                                      \cdashline{2-7}[5pt/1pt]
                                   &\underline{ \textbf{CO$_2$-Net \cite{hong2021cross}}}           & \textbf{ACM MM 2021}           & \textbf{43.3} & \textbf{26.3} & \textbf{5.2} & \textbf{26.4} \\
                                      & \textbf{CO2-Net+NoCo}            & \textbf{-}                     & \textbf{48.9} & \textbf{30.0}   & \textbf{6.6} & \textbf{30.1} \\
                                      \cdashline{2-7}[5pt/1pt]
                                       &  \underline{\textbf{ASM-Loc \cite{he2022asm}}}         & \textbf{CVPR 2022}              & \textbf{43.4} & \textbf{26.6} & \textbf{5.3} & \textbf{26.5} \\
                                      & \textbf{ASM-Loc+NoCo}            & \textbf{-}                     & \textbf{49.1} & \textbf{30.5} & \textbf{6.7} & \textbf{30.7} \\ 
                                      \hline
    \end{tabular}
}
\label{new-table2}
\end{table}

==> table/NoName-0725.tex <==
\begin{table}[htb]
\centering
\caption{caption title todo}
\renewcommand\arraystretch{1.2}
\resizebox{\linewidth}{!}{

\begin{tabular}{c|cc|ccccc}
\hline
                                   &                                        &                                  & \multicolumn{4}{c}{\textbf{mAP@IoU(\%)}}                                                                                  & \textbf{AVG}                 \\ \cline{4-8} 
\multirow{-2}{*}{\textbf{Dataset}} & \multirow{-2}{*}{\textbf{Method}}      & \multirow{-2}{*}{\textbf{Pub.}}  & 0.1                          & 0.3                          & 0.5                          & 0.7                          & (0.1:0.7)                    \\ \hline
                                   & SF-Net{[}36{]}                         & ECCV2020                         & 58.0                         & 37.9                         & 19.3                         & 11.9                         & 31.0                         \\
                                   & DCM{[}37{]}                            & ICCV2021                         & 59.7                         & 38.3                         & 21.9                         & 18.1                         & 33.7                         \\
                                   & PCL{[}42{]}                            & ESWA2023                         & 65.2                         & 56.8                         & 34.3                         & 21.2                         & 44.9                         \\
                                   & Li et al.{[}62{]}                      & CVPR2021                         & 60.2                         & 44.7                         & 28.8                         & 12.2                         & 36.4                         \\ \cline{2-8} 
                                   & \cellcolor[HTML]{D9D9D9}LACP{[}43{]}   & \cellcolor[HTML]{D9D9D9}ICCV2021 & \cellcolor[HTML]{D9D9D9}63.9 & \cellcolor[HTML]{D9D9D9}55.7 & \cellcolor[HTML]{D9D9D9}33.9 & \cellcolor[HTML]{D9D9D9}20.8 & \cellcolor[HTML]{D9D9D9}43.5 \\
                                   & \cellcolor[HTML]{D9D9D9}LACP+NoCo      & \cellcolor[HTML]{D9D9D9}-        & \cellcolor[HTML]{D9D9D9}66.5 & \cellcolor[HTML]{D9D9D9}58.2 & \cellcolor[HTML]{D9D9D9}36.5 & \cellcolor[HTML]{D9D9D9}21.2 & \cellcolor[HTML]{D9D9D9}46.1 \\
                                   & \cellcolor[HTML]{D9D9D9}HR-Pro{[}44{]} & \cellcolor[HTML]{D9D9D9}AAAI2024 & \cellcolor[HTML]{D9D9D9}72.6 & \cellcolor[HTML]{D9D9D9}61.1 & \cellcolor[HTML]{D9D9D9}37.3 & \cellcolor[HTML]{D9D9D9}17.5 & \cellcolor[HTML]{D9D9D9}47.3 \\
\multirow{-8}{*}{\textbf{GTEA}}    & \cellcolor[HTML]{D9D9D9}HR-Pro+NoCo    & \cellcolor[HTML]{D9D9D9}-        & \cellcolor[HTML]{D9D9D9}74.0 & \cellcolor[HTML]{D9D9D9}62.4 & \cellcolor[HTML]{D9D9D9}39.0 & \cellcolor[HTML]{D9D9D9}19.1 & \cellcolor[HTML]{D9D9D9}48.6 \\ \hline
                                   & SF-Net{[}36{]}                         & ECCV2020                         & 62.9                         & 40.6                         & 16.7                         & 3.5                          & 30.9                         \\
                                   & DCM{[}37{]}                            & ICCV2021                         & 63.2                         & 46.8                         & 20.9                         & 5.8                          & 34.9                         \\
                                   & BackTAL{[}40{]}                        & TPAMI2021                        & 60.1                         & 40.9                         & 21.2                         & 11.0                         & 32.5                         \\
                                   & PCL{[}42{]}                            & ESWA2023                         & 78.7                         & 63.3                         & 44.1                         & 26.9                         & 53.3                         \\
                                   & Li et al.{[}62{]}                      & CVPR2021                         & 71.5                         & 40.3                         & 20.3                         & 5.5                          & 34.4                         \\ \cline{2-8} 
                                   & \cellcolor[HTML]{D9D9D9}LACP{[}43{]}   & \cellcolor[HTML]{D9D9D9}ICCV2021 & \cellcolor[HTML]{D9D9D9}76.9 & \cellcolor[HTML]{D9D9D9}61.4 & \cellcolor[HTML]{D9D9D9}42.7 & \cellcolor[HTML]{D9D9D9}25.1 & \cellcolor[HTML]{D9D9D9}51.8 \\
                                   & \cellcolor[HTML]{D9D9D9}LACP+NoCo      & \cellcolor[HTML]{D9D9D9}-        & \cellcolor[HTML]{D9D9D9}80.2 & \cellcolor[HTML]{D9D9D9}64.9 & \cellcolor[HTML]{D9D9D9}46.1 & \cellcolor[HTML]{D9D9D9}26.9 & \cellcolor[HTML]{D9D9D9}55.1 \\
                                   & \cellcolor[HTML]{D9D9D9}HR-Pro{[}44{]} & \cellcolor[HTML]{D9D9D9}AAAI2024 & \cellcolor[HTML]{D9D9D9}78.5 & \cellcolor[HTML]{D9D9D9}72.1 & \cellcolor[HTML]{D9D9D9}55.3 & \cellcolor[HTML]{D9D9D9}26.1 & \cellcolor[HTML]{D9D9D9}59.4 \\
\multirow{-9}{*}{\textbf{BEOID}}   & \cellcolor[HTML]{D9D9D9}HR-Pro+NoCo    & \cellcolor[HTML]{D9D9D9}-        & \cellcolor[HTML]{D9D9D9}78.6 & \cellcolor[HTML]{D9D9D9}72.3 & \cellcolor[HTML]{D9D9D9}55.6 & \cellcolor[HTML]{D9D9D9}26.2 & \cellcolor[HTML]{D9D9D9}59.6 \\
\hline
\end{tabular}%

}
\label{new-table2}
\end{table}
